FwdLLM: Efficient FedLLM using Forward Gradient

Large Language Models (LLMs) are transforming the landscape of mobile intelligence. Federated Learning (FL), a method to preserve user data privacy, is often employed in fine-tuning LLMs to downstream mobile tasks, an approach known as FedLLM. Though recent efforts have addressed the network issue induced by the vast model size, they have not practically mitigated vital challenges concerning integration with mobile devices, such as significant memory consumption and sluggish model convergence. In response to these challenges, this work introduces FwdLLM, an innovative FL protocol designed to enhance the FedLLM efficiency. The key idea of FwdLLM to employ backpropagation (BP)-free training methods, requiring devices only to execute ``perturbed inferences''. Consequently, FwdLLM delivers way better memory efficiency and time efficiency (expedited by mobile NPUs and an expanded array of participant devices). FwdLLM centers around three key designs: (1) it combines BP-free training with parameter-efficient training methods, an essential way to scale the approach to the LLM era; (2) it systematically and adaptively allocates computational loads across devices, striking a careful balance between convergence speed and accuracy; (3) it discriminatively samples perturbed predictions that are more valuable to model convergence. Comprehensive experiments with five LLMs and three NLP tasks illustrate FwdLLM's significant advantages over conventional methods, including up to three orders of magnitude faster convergence and a 14.6x reduction in memory footprint. Uniquely, FwdLLM paves the way for federated learning of billion-parameter LLMs such as LLaMA on COTS mobile devices -- a feat previously unattained.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> alg-forward-fl.tex <==
\begin{algorithm}[t]
	\footnotesize
	\SetAlgoNoEnd
  \SetKwProg{Fn}{Function}{~}{end}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      Pre-trained model, $\Theta$;\\
      Target accuracy, $acc$.
    }

  \Output{
      Fine-tuned model, $\Theta_{i}$~(i=1,2\dots).
      % $Q_b$\;   
    }
  \BlankLine

  \Fn{Cloud\_controller():}{
    Iteration $i$=0, Model $\Theta_{i}$=$\Theta$; // initial\\
    % $l_{win}$, $l_{candidate}$, $i$ $\leftarrow$ Switch($i,l$); // initial pace configuration\\
    % $Client_{train}$ $\leftarrow$ selects $N$ clients;\\
    % Iteration i=0;\\
      \While{Eval($\Theta_{i}$) $<$ $acc$}
      { 
        Generate random seeds $S_{i}$;\\
        Send $\Theta_{i}$ and $S_{i}$ to clients;\\
        Wait;\\
        $\nabla_v f(\theta)$ $\leftarrow$ Directional derivatives from clients;\\
        perturbations $V_{i}$ $\leftarrow$ seed $S_{i}$;\\
        $g_{v}(\theta)$ $\leftarrow$ $\nabla_v f(\theta)$v;\\
        $g_{i}$ $\leftarrow$ Aggregate($g_{v}(\theta)$);\\
        $\Theta_{i+1}$ $\leftarrow$ $\Theta_{i}$ - $\eta g_{i}$;\\
        $i$ $\leftarrow$ $i$ + 1;\\
        }
        Exit training.
      }

    \Fn{Client\_training(i):}{
        Receive $\Theta_{i}$ and $S_{i}$ from cloud;\\
        perturbations $V_{i}$ $\leftarrow$ seed $S_{i}$;\\
        $\nabla_v f(\theta)$ $\leftarrow$ compute directional derivatives via Equation~\ref{eq:directional-derivative};\\
        Send $\nabla_v f(\theta)$ to cloud.
    }

  \caption{Forward-only FedLLM}\label{alg:forward-fl}
\end{algorithm}


==> fig-design-adaption-equal.tex <==
\begin{figure}[t]
	\centering
    \includegraphics[width=0.30\textwidth]{figs/design-adaptation-equal.pdf}
    \caption{Adding clients and adding local perturbations are equivalent in terms of the number of samples.}
	\label{fig:design-adaptation-equal}
\end{figure}

==> fig-design-peft-params.tex <==
\begin{figure}[t]
	\centering
    \includegraphics[width=0.30\textwidth]{figs/design-peft-params.pdf}
    \caption{Correlation between clients and tunable parameters. \cdq{Linearly or exponentially?}. Dataset: \cdq{XXX}. Model: \cdq{XXX}.}
	\label{fig:design-peft-params}
\end{figure}

==> fig-eval-ablation-adaptive.tex <==
\begin{figure}[htbp]
	\centering
    \includegraphics[width=0.23\textwidth]{figs/eval-ablation-adaptive.pdf}
    \caption{Adaptive vs Fixed. Model:Distilbert. Dataset:AGNews}
	\label{fig:eval-ablation-adaptive}
\end{figure}

==> fig-eval-llama.tex <==
\begin{figure}[t]
	\centering
    \includegraphics[width=0.23\textwidth]{figs/eval-llama-agnews.pdf}
    \caption{the performance of \sys on LLaMA. 
    % \cdq{Change the axis to real runtime (quantized). 
    % The meta-data could be taken from MobileFM (in new Jetson board).
    % The baseline is backpropagation training in NVIDIA A100.
    % Forward-FL BS = 8.
    % Client = 100.
    % LR = 3e-4.}

    % \wyz
    % forward 
    % 学习率用的是3e-3，bs=8，client num = 100
    % 每个batch的时间： 0.74*2+4.2/10   (0.74s infer一次，参数量4.2M，带宽10MB) (突然发现这里需要再确认一下参数量，是4.2M个参数还是4.2MB)
    % 每20个batch test一次，test acc如下
    % 0, 0, 0, 0.555, 0.78, 0.825, 0.825, 0.85, 0.855, 0.855, 0.855, 0.87, 0.87, 0.875, 0.875, 0.875, 0.88, 0.88, 0.88, 0.88, 0.88, 0.88, 0.88, 0.88, 0.89, 0.89, 0.895, 0.895, 0.895, 0.9, 0.9, 0.9, 0.9, 0.9, 0.905, 0.905,
    % 600个batch能到0.9准确率
    }

	\label{fig:eval-llama-agnews}
\end{figure}

==> fig-eval-model-bert-large.tex <==
\begin{figure}[t]
	\centering
    \includegraphics[width=0.23\textwidth]{figs/eval-model-bert-large.pdf}
    \caption{BERT-Large.}
	\label{fig:eval-model-bert-large}
\end{figure}

==> fig-eval-niid.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        % \begin{minipage}[b]{0.24\textwidth}
        %     \includegraphics[width=1\textwidth]{figs/eval-niid-albert-agnews.pdf}
        % \end{minipage}
        % ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/eval-niid-distilbert-agnews.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/eval-niid-bert-agnews.pdf}
        \end{minipage}
        % ~
        % \begin{minipage}[b]{0.24\textwidth}
        %     \includegraphics[width=1\textwidth]{figs/eval-niid-roberta-large-agnews.pdf}
        % \end{minipage}
        % \subcaption{\texttt{AGNEWS}}
    \end{minipage}

    \caption{the performance of \sys on non-iid data distribution}
    \label{fig:eval-niid}
\end{figure}

==> fig-eval-privacy.tex <==
\begin{figure}[t]
	\centering
    \includegraphics[width=0.40\textwidth]{figs/eval-privacy.pdf}
    \caption{\sys is easy to be integrated with other privacy-preserving protocols.}
	\label{fig:eval-privacy}
\end{figure}

==> fig-eval-quant-llama.tex <==
\begin{figure}[t]
	\centering
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1\textwidth]{figs/eval-quant.pdf}
        \subcaption{\sys performance after quantization. 
        \cdq{Change the axis to real-time (especially for int-plot).}
        }
        \label{fig:eval-quant}
    \end{minipage}~
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1\textwidth]{figs/eval-llama-agnews.pdf}
        \subcaption{Performance of \sys on LLaMA. \cdq{Clients for \sys: \cdq{100}.
        % clients for backward: 1.
        }
        % \mwx{numbers seem weird. how it's measured?}
        }
        \label{fig:eval-llama-agnews}
    \end{minipage}
    \caption{\sys is scalable to large models.}
\end{figure}

% \begin{figure}[t]
% 	\centering
%     \includegraphics[width=0.23\textwidth]{figs/eval-e2e-clients.pdf}
%     % 这里fedavg和fedsgd用的其实是bert模型，distilbert等后续重跑
%     \caption{End-to-end performance under different involved clients. 
%     % \cdq{Remove fedavg results to avoid confusion. Include baselines results.}
%     }
% 	\label{fig:eval-model-bert-large}
% \end{figure}

% \begin{figure}[t]
% 	\centering
%     \includegraphics[width=0.23\textwidth]{figs/eval-llama-agnews.pdf}
%     \caption{the performance of \sys on LLaMA. 
%     % \cdq{Change the axis to real runtime (quantized). 
%     % The meta-data could be taken from MobileFM (in new Jetson board).
%     % The baseline is backpropagation training in NVIDIA A100.
%     % Forward-FL BS = 8.
%     % Client = 100.
%     % LR = 3e-4.}
%     }

% 	\label{fig:eval-llama-agnews}
% \end{figure}

==> fig-intro-framework.tex <==
\begin{figure}[t]
	\centering
    \includegraphics[width=0.49\textwidth]{figs/intro-framework.pdf}
    \caption{Classic and forward-only federated learning. \mwx{can be removed}}
	\label{fig:intro-framework}
\end{figure}

==> fig-motivations.tex <==
\begin{figure}[t]
	\centering
        \begin{minipage}[b]{0.48\textwidth}
            \includegraphics[width=1\textwidth]{figs/design-pitfall-memory.pdf}
            \subcaption{Memory. BS: 8. Sequence length: 256.}
        \end{minipage}

        
        \begin{minipage}[b]{0.48\textwidth}
            \begin{minipage}[b]{0.48\textwidth}
            \includegraphics[width=1\textwidth]{figs/design-pitfall-clients-agnews-adapter.pdf}
            \subcaption{Clients (w/ adapter)}
            \end{minipage}~
            \begin{minipage}[b]{0.48\textwidth}
                \includegraphics[width=1\textwidth]{figs/design-pitfall-clients-agnews.pdf}
                \subcaption{Clients (w/o adapter)}
            \end{minipage}
        \end{minipage}

    \caption{Pitfalls of backprop-based FL. \mwx{Why FedSGD? Shall be FedAvg.}}
	\label{fig:motivations}
\end{figure}



==> sec-design-math.tex <==
%\subsection{Forward-only Federated Learning}
%\label{sec:design-math}

\paragraph{Forward Gradients}
\mwx{need to be improved}
\cdq{I have polished the sentences, any other suggestions?}
Here, we provide a brief introduction to the mathematical basis of forward gradients.
To compute the directional derivatives of deep learning functions, denoted as \(f\), with respect to a vector \(v\) at a point \(\theta\), the following equation can be used~\cite{rumelhart1985learning, lecun2015deep}:
\begin{equation}
    \nabla_v f(\theta) = \lim _{h \rightarrow 0} \frac{f(\theta+h \cdot v) - f(\theta)}{h},
    \label{eq:directional-derivative}
\end{equation}
where \(v \in N(0,1)\) represents the weight perturbations, and \(\nabla_v f(\theta)\) is the directional derivative of \(f\) at the model weight point \(\theta\) in the direction \(v\)~\cite{deisenroth2020mathematics}.
In simpler terms, \(\nabla_v f(\theta)\) signifies the slope of \(f\) in the direction of \(v\).
The direction of steepest ascent can be identified using the gradient \(\nabla f(\theta)\).
Nevertheless, determining the gradient \(\nabla f(\theta)\) can be computationally demanding, as it necessitates both a forward pass and a backward pass~\cite{baydin2022gradients}, which we have empirically validated in Section~\ref{sec:bkgnd}.
As an alternative, we leverage the forward gradient \(g_{v}\), which is more cost-effective to compute:
\begin{equation}
    g_v(\theta) := \nabla_v f(\theta) v = (\nabla f(\theta) \cdot v) v,
    \label{eq:forward-gradient}
\end{equation}
where \(g_v(\theta)\) is established as an unbiased estimator of the gradient \(\nabla f(\theta)\)~\cite{baydin2022gradients}.

% Forward gradient allows us to compute $\nabla f(\theta)$ by evaluating $f$ forward $n$ times with direction vectors $v$ taken as standard Gaussian $N(0,1)$.
% \mwx{Compress the above by around 1/3. Give rationales.}

Using Figure~\ref{fig:design-forward-effectiveness-samples} as an illustrative example, we demonstrate the computation of gradients for the function \(z=2(x^2+y^2)\) at the point \((0,0.5)\).
We can sample \(n\) direction vectors \(v\) from \(N(0,1)\) and compute \(g_v(\theta)\) for each \(v\). By taking the average of these forward gradients \(g_v(\theta)\), we obtain an estimator for the true (backward) gradient \(\nabla f(\theta)\).
% \mwx{What model? Need more details.}

\cdq{Directly applying forward gradients to LLMs will lead to overfitting or necessities of billion size clients/perturbations involved.
We find that the training complexity is primarily related to teh trainable parameter size instead of the total size.
We propose to leverage 
}
\paragraph{Rationales behind forward gradients-based FedLLM}
Although forward gradients have been proposed in previous literature~\cite{barto1987gradient,hinton2022forward,ma2020hsic, baydin2022gradients, sun2022bbtv2,park2023fedfwd}, their practical application has been limited, primarily due to the enormous data and computational demands. Specifically, the requirements (i.e., perturbations per batch) are exponentially proportional to the parameter size.
Prior forward gradients research has been restricted to evaluations on small-scale models such as LeNet and VGG-9~\cite{baydin2022gradients,ren2022scaling, park2023fedfwd}.
\sys represents the first attempt to apply forward gradient methodology to FedLLM, guided by two underlying rationales:
(1) Through extensive offline experiments, we observe that the training complexity is primarily related to the \textit{trainable} parameter size, rather than the total size~\cite{baydin2022gradients,ren2022scaling, park2023fedfwd}. This observation is intuitively consistent with the mathematical foundation expressed as $f(\theta | \Theta, x)$, where the pre-trained model weight $\Theta$ and input $x$ remain fixed, with only the PEFT weights $\theta$ being tunable. Fortunately, pre-trained LLMs have accumulated rich generic knowledge, thus requiring only a small number of new parameters to adapt to various downstream tasks.
%This adaptation refers to the process of federated learning with PEFTs, where the larger the LLM, the fewer trainable parameters are needed for each task.
(2) Mobile devices possess significant scalability, allowing for the simultaneous computation of forward gradients.

\begin{comment}
\mwx{Not needed?}
\cdq{I think we should upload directional derivative instead of gradients. Because: 1) our network cost is not good enough; 2)lora of LLaMa is about 4MB, uploading gradients is too heavy.
So this part is important to state the different between traditional FL.}
\input{alg-forward-fl.tex}
Algorithm~\ref{alg:forward-fl} describes how \sys leverages forward gradient to train LLMs in a federated manner.
First, server sends model parameters and random seeds to clients (line 1--5). Different clients will be dispatched different seeds, noted as $S_{i} = \{s_{i}^{k}\}$ for $client_{i}$;
Then, clients generate perturbations $v_{i}^{k}$ for each seed $s_{i}^{k}$ (line 15--16); 
Next, clients compute directional derivative $\nabla_v f(\theta)$ for each $v_{i}^{k}$ using Equation~\ref{eq:directional-derivative} (line 17);
Clients upload directional derivative $\nabla_v f(\theta)$ to server (line 18). 
Noted that $\nabla_v f(\theta)$ is a scalar, which is much smaller than the model parameters;
Server generates perturbations $v_{i}^{k}$ for each seed $s_{i}^{k}$ as clients and compute forward gradients $g_{v_{i}^{k}}(\theta)$ using Equation~\ref{eq:forward-gradient}, then aggregate forward gradients $g_{v}(\theta)$ from all clients (line 7--11).
Step 1--5 are repeated for each round of federated learning until the model converges.
\end{comment}
\input{fig-design-forward-fl-memory.tex}

\noindent \textbf{\sys's advantages by design.}
(1) \sys is computationally efficient. For each client, calculating a forward gradient is equivalent to executing inferences twice (i.e., $f(\theta+h \cdot v)$ and $f(\theta)$), making its execution on NPU 19.5--27.5$\times$ faster than computing one backward gradient on a CPU, as previously demonstrated in Table~\ref{tab:motivations-latency}.
(2) \sys is memory-efficient, as it does not require storage of the intermediate activations generated during the forward pass, which contribute to the majority of the memory footprint, as outlined in $\S$\ref{sec:back:exps}. The perturbation weights are parameter-efficient, and the perturbed LLM can be generated sequentially, with each being immediately released once its inference is completed (Figure~\ref{fig:design-forward-fl-memory}). Thus, the peak memory footprint of \sys can be approximated as $size\_of(\mathcal{M})+2 \cdot trainable\_param$.
(3) \sys is highly scalable with respect to client numbers. As more clients compute forward gradients simultaneously, the aggregated gradient becomes closer to the real gradient, contributing to faster and more accurate convergence. Figure~\ref{fig:design-forward-effectiveness-statistics} illustrates that the continuous addition of perturbations enables the forward gradients to estimate the true gradient with greater precision and stability.

\paragraph{Forward gradients with PEFT}
Forward gradient is orthogonal to different PEFT methods.
\sys lets the developers to choose a PEFT method, yet can also provide heuristics-based recommendations for FL developers in choosing a proper PEFT method based on the LLM size, client number, and private training dataset size.
Generally, larger LLM and less clients/data favor more aggressive PEFT methods (e.g., BitFit and LoRa) that result in less trainable parameters.

\begin{comment}
\paragraph{Computation cost analysis}
According to Equation~\ref{eq:forward-gradient}, the forward gradient $g_{v}(\theta)$ is computed by multiplying the directional derivative $\nabla_v f(\theta)$ with the perturbation vector $v$, where $\nabla_v f(\theta)$ is computed via Equation~\ref{eq:directional-derivative}.
Since cloud is aware of the perturbation vector $v$, the multiplication can be done on cloud.
In conclusion, from client perspective, calculating a forward gradient equals to running two inference, i.e., $f(\theta+h \cdot v)$ and $f(\theta)$.
The time cost of running two inference is \cdq{XX-XX}$\times$ faster than computing one backward-gradients, as we have shown in Table~\ref{tab:motivations-latency}.
\end{comment}

% \mwx{
% have a paragraph to summarize how forward gradient differs from inference, from the computation perspective. For example:    
% From the computing perspective, calculating a forward gradient equals to running inference with a certain batch size and XXX.}


\input{fig-design-forward-effectiveness.tex}

==> sec-eval-niid.tex <==
\subsection{Non-iid Data Distribution}
\label{sec:eval-niid}




==> sec-eval-privacy.tex <==
\subsection{Conjunction with privacy-preserving protocols}
\label{sec:eval-privacy}
\input{fig-eval-privacy.tex}


As shown in Fig.~\ref{fig:eval-privacy}, we integrate \sys with four privacy-preserving protocols mentioned above to evaluate the runtime performance.


==> sec-measurement.tex <==
\subsection{Experimental Observations}\label{sec:measurement}


==> tab-design-planning-configuration.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|c|ccccc|}
    \hline
    \multirow{2}{*}{Models} & \multirow{2}{*}{Task} & \multicolumn{5}{c|}{Relative Conv. Acc}                                                                              \\ \cline{3-7} 
                            &                       & \multicolumn{1}{c|}{99\%} & \multicolumn{1}{c|}{95\%} & \multicolumn{1}{c|}{90\%} & \multicolumn{1}{c|}{80\%} & 60\% \\ \hline
    DISTILBERT                    & AGNEWS                & \multicolumn{1}{c|}{50}   & \multicolumn{1}{c|}{10}    & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{3}    & 3    \\ \hline
    ...                     & ...                   & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     &      \\ \hline
    \end{tabular}%
    }
    \caption{Best Global-PS configuration towards different relative convergence accuracy.}
    \label{tab:design-planning-configuration}
    \end{table}

==> tab-eval-overall-cpu.tex <==
\begin{table*}[t]
	\scriptsize
    \includegraphics[width=17cm]{figs/tab-eval-e2e-cpu.pdf}
\caption{End-to-end performance evaluation. Device: Intel Core XX CPU @ XXHz.}
\label{tab:eval-e2e-cpu}
\end{table*}


==> tab-eval-overall-npu.tex <==
\begin{table*}[t]
	\scriptsize
    \includegraphics[width=17cm]{figs/tab-eval-e2e-npu.pdf}
\caption{End-to-end performance evaluation. Device: Google Pixel 7P (XX). }
\label{tab:eval-e2e-npu}
\end{table*}


==> tab-impl-setup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]

    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|l|l|l|cl|}
    \hline
    \multirow{2}{*}{Model} & \multirow{2}{*}{Dataset} & \multirow{2}{*}{PEFT Algo.} & \multicolumn{2}{c|}{Memory usage (GB)}                                             \\ \cline{4-5} 
                           &                          &                             & \multicolumn{1}{c|}{Backpropagation-based FL} & \multicolumn{1}{c|}{FedFWD (ours)} \\ \hline
    DistilBERT-base        & AGNEWS                   & Adapter                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}              \\ \hline
    DistilBERT-base        & YAHOO                    & Adapter                     & \multicolumn{1}{l|}{}                         &                                    \\ \hline
    BERT-large             & AGNEWS                   & Bias-tuning                 & \multicolumn{1}{l|}{}                         &                                    \\ \hline
    \end{tabular}%
    }
    \caption{Evaluation setups.}
    \label{tab:eval-setup}
    \end{table}

==> todo.tex <==
\mwx{term: unlabeled data}

\mwx{Curriculum Learning: from easy samples to difficult ones. Our system: from easy model to difficult ones.}

\mwx{cloud service or aggregator?}
